Generative Models: An Interdisciplinary Perspective

By linking conceptual theories with observed data, generative models can support reasoning in complex situations. They have come to play a central role both within and beyond statistics, providing the basis for power analysis in molecular biology, theory building in particle physics, and resource allocation in epidemiology, for example. We introduce the probabilistic and computational concepts underlying modern generative models and then analyze how they can be used to inform experimental design, iterative model refinement, goodness-of-fit evaluation, and agent-based simulation. We emphasize a modular view of generative mechanisms and discuss how they can be flexibly recombined in new problem contexts. We provide practical illustrations throughout, and code for reproducing all examples is available at https://github.com/krisrs1128/generative_review. Finally, we observe how research in generative models is currently split across several islands of activity, and we highlight opportunities lying at disciplinary intersections.

==> UsefulPackages.tex <==
Bioinformatics:
scDesign
seqgen
splatter
MSstatsSampleSize
PROPER
MOSim



https://cran.r-project.org/web/views/ExperimentalDesign.html

acebayes
adaptDiag	Bayesian Adaptive Designs for Diagnostic Trials
ADCT	Adaptive Design in Clinical Trials
adoptr	Adaptive Optimal Two-Stage Designs in R
adpss	Design and Analysis of Locally or Globally Efficient Adaptive Designs
agricolae	Statistical Procedures for Agricultural Research
agricolaeplotr	Visualization of Design of Experiments from the 'agricolae' Package
AlgDesign	Algorithmic Experimental Design
ALTopt	Optimal Experimental Designs for Accelerated Life Testing
Aoptbdtvc	A-Optimal Block Designs for Comparing Test Treatments with Controls
asd	Simulations for Adaptive Seamless Designs
bacistool	Bayesian Classification and Information Sharing (BaCIS) Tool for the Design of Multi-Group Phase II Clinical Trials
BayesCR	Bayesian Analysis of Censored Regression Models Under Scale Mixture of Skew Normal Distributions
bayesCT	Simulation and Analysis of Adaptive Bayesian Clinical Trials
BayesDesign	Bayesian Single-Arm Design with Survival Endpoints
BayesPPD	Bayesian Power Prior Design
BDEsize	Efficient Determination of Sample Size in Balanced Design of Experiments
bdlp	Transparent and Reproducible Artificial Data Generation
bioOED	Sensitivity Analysis and Optimum Experiment Design for Microbial Inactivation
deepgp	Sequential Design for Deep Gaussian Processes using MCMC
DelayedEffect.Design	Sample Size and Power Calculations using the APPLE and SEPPLE Methods
demu	Optimal Design Emulators via Point Processes

DiceDesign	Designs of Computer Experiments
DiceKriging	Kriging Methods for Computer Experiments

DiceOptim	Kriging-Based Optimization for Computer Experiments

earlyR	Estimation of Transmissibility in the Early Stages of a Disease Outbreak

easypower	Sample Size Estimation for Experimental Designs

experDesign	Design Experiments for Batches

faux	Simulation for Factorial Designs

FielDHub	A Shiny App for Design of Experiments in Life Sciences

FieldSim	Random Fields (and Bridges) Simulations

geospt	Geostatistical Analysis and Design of Optimal Spatial Sampling Networks

gscounts	Group Sequential Designs with Negative Binomial Outcomes

hiPOD	hierarchical Pooled Optimal Design
MCPModPack	Simulation-Based Design and Analysis of Dose-Finding Trials


==> purgatory.tex <==

% this is for material that we don't want to delete forever but which probably shouldn't be included in the draft


From introduction,

A simple way of teaching complex statistical ideas is to generate data with a known model and see how the analytical
methods work on the simulated data. This is standard use in
teaching mixture models\citep{HolmesHuber}, latent variable models or  and in calibrating new methods
(see examples \cite{slatkin1996testing}). This method is necessary 
because it is impossible to understand a new method on complex unknown data. Generative methods, or the "top down" approach have been used in probabilistic modeling before the use of computers(for an example see the study of mixtures and their generation in \cite{Teicher1960mixture}) and at the very onset of the Monte Carlo revolution (\cite{metropolis1949monte}). 
This early use of simulation based generative methods has matured into  methods that
 can accommodate unknown normalizing constants through Gibbs sampling, Approximate Bayesian methods for unknown
 densities 
and simulator-based statistical model fitting. 
Key in these approaches is the iterative comparison
between simulated data and the inferred probabilistic model using
various measures of discrepancy. 

Today the generative approach dominates the methodological landscape of calibration and design of experiments, likelihood free inference,  data modelling and decision making under uncertainty. 

At early stages of the scientific process, generative models are also invaluable communication tools. For instance
when illustrating notions of identifiability to collaborators, simulation of different scenarios can show indistinguishability of the different outputs, thus elucidating sources of non-identifiability\citep{brun2001practical}. 

At the other end of the specification spectrum, many scientific communities, economics, biology and  physics have refined bottom-up generative models, often called "Agent Based Models" (ABM),  deterministic approximations that
simulate complex systems by identifying interactions between large numbers of similar agents. Such models have been used for modeling disease dynamics and we will show how they can be used to infer mutation rates in butterflies and have assisted policy makers during Covid. 

Simulations relieve the researcher from needing full distributional specifications, procedures based on optimization and simulation minimize discrepancies 
between model and data when complete densities 
are unavailable. These proceed by adaptive
probabilistic modeling. An example of such a strategy using Bayesian optimization is developed in \cite{gutmann2016bayesian}.

The methods for using these models for inference are Section \ref{sec:inference}.


Section \ref{sec:calibration} covers goodness of fit and discrepancy measures.
We provide an example of using statistical learning to do a semi-automatic evaluation of
the quality of the  model approximations.
In section \ref{sec:emulation}  we show several examples where  these
methods enable the
the study of complex systems, such as adaptive evolution and epidemics.
Finally, the conclusion outlines some of the ideas that are driving current progress in the field, these originate from many different communities and we highlight the interdisciplinary future challenges
that will benefit scientists and policy makers.



From Conclusion,


%%%%What is missing? Challenges??
%%%%Challenges: a stab at it...

In all of generative models we have exemplified, we are confronted with the problem of choosing the
right "levels of approximation".
In ABMs for example,  we pretend we know the attributes of the agents
but have to leave out a lot of the details, making the agents more partially exchangeable than they really are. In variational methods we use local expectations instead of the full
densities, computational constraints and lack of full knowledge force
use to approximate, the question then becomes:
does it matter? It is obvious that the data themselves have enough variability that once we can make an approximate model that generates data that is indistinguishable from the real data, our approximation is "good enough". Again the measure of discrepancy that says the data are indistinguishable from the model is the essential component.

Recent theoretical work on using Stein kernels\cite{gorham2019measuring} and optimal transport\cite{solomon2015convolutional} as
tools for measuring discrepancies are appearing side by side with
the Adverserial Network type approaches initiated in \cite{friedman2003}.
As one can see, many challenges still exist in the interpretation of the discrepancies and their iterative minimization.

Generative models are used by multiple separate communities. We've mentioned physicists, economists, epidemiologists, behavioral ecologists, biostatisticians and computer scientists. 
Even the least data oriented scientists such as mathematicians~\cite{mazur2008finding} are using generative models to generate and refine conjectures. However, there are difficulties in
leveraging methods across fields, mostly due to cultural habits and
language.

A recent review\cite{cranmer_frontier_2020} covers the extensive progress of generative models used in deep learning. 
As pointed out in a recent review~\cite{baker2022analyzing}, ABM can be streamlined by using statistical methods and proxies such as Gaussian Processes. These smoothing approximations provide a path to tractability: the path between ABM and statistical methods is a continuum, where hierarchical approximations can improve tractability issues while accounting for the granular heterogeneity when the "agent-particles" are   not perfectly exchangeable.
In the other direction, much success in Bayesian posterior computations was attained when statisticians reversed the smoothing process and went from densities to point mass distributions over populations of particles, in methods we now know as particle filters. In fact, nonlinear extensions of the Kalman filter where probability distributions are simulated at discrete points that multiply and reweight themselves (see the classic review by \cite{doucet2001introduction}). 

Progress in combining granular and smooth approaches has been intense during the covid pandemic where decision making had to be simulation based until data could complement the process. Climate and studies of ecological change will continue to be dependent on generative models.





It is encouraging to see so much of the code and work done by groups become quickly available through open source computational
resources. Reproducibility and cross-disciplinary vocabulary will continue to enhance this exponentially growing field.



%Here are a few examples:
%\begin{description}
%\item[Non-identifiability and sloppiness]
%In systems biology, a common theme is the robustness of parametrizations of complex systems, this is often referred to as
%sloppiness\cite{gutenkunst2007universally}, statisticians are more familiar with the parallel notion of non-identifiability.
%\item[Linearity and non-linearity]
%Statisticians use the term "nonlinear" for cases where the relationships between variables are not linear. In biophysics, genetics and
%economics, complex phenomenon which have discontinuities or chaotic
%behaviors are said to be {\it nonlinear}. They are often studied through 
%\item[Variational approximations at different granularities]
%Analytical approximations instead of MCMC, another such approximation is INLA
%\end{description}






\subsection{Simulation based discoveries}
%%%%Maybe this could go into the conclusion
Computational generative models are now the 
main instrument for modern statistics even in theory we
have experimental evidence for new conjectures generated

\cite{bertsimas2020sparse}
\cite{bertsimas2016best}
\cite{hastie2020best}



Other title ideas

Generative Models: A Review of Methods and Applications
Generative Models for Decision making
Guiding Decisions through Generative Models
Generative Models: An Interdisciplinary Perspective
Guiding Decisions through Generative Models: An Interdisciplinary Review
Generative Models: An Interdisciplinary View of Methods and Applications



\subsubsection{Simulation as computation with units}

In all the examples above, we were interested in the global, long-term properties of a system, but it was easier to reason about how they change locally and immediately. Simulation helps bridge these scales, applying brute force computation to clarify high-level structure by unrolling the behavior of elementary, interacting units. 
This was useful both for direct modeling and for indirect inference. The elementary units can be agents in an Agent Based Model or particles in Sequential Monte Carlo. For example, we saw agents used to analyze properties of long-run disease trajectories and particles used to guide inference about a population parameter (mutation rate).


Other idea: At the "observation" level, instead of generating data from scratch, we often use simulations to increase data sizes by "jittering" (as in NN), by resampling (as in boosting and bagging).

The underlying generative model to think about there is the Bayesian
prior for the data and parameters, ie the way ridge regression can be understood as the Bayesian approach where the coefficients are Normal random variables is equivalent to 



Other idea, I don't know where to include it but I wanted to mention 
"levels of approximation".

In ABM for instance, we pretend we know the attributes of the agents
but have to leave out a lot of the details.
In variational methods we use local expectations instead of the full
densities, computational constraints and lack of full knowledge force
use to approximate, the question then becomes:
does it matter?
It is obvious that the data themselves have enough variability that
once we can make an approximate model that generates data that is
indistinguishable from the real data, our approximation is "good enough".






%\subsection{Reproducibility of COVID-19 simulators}

\url{https://www.ebi.ac.uk/biomodels/covid-19}

